Benchmarking Robustness of Adaptation Methods on Pre-trained Vision-Language Models

Various adaptation methods, such as LoRA, prompts, and adapters, have been proposed to enhance the performance of pre-trained vision-language models in specific domains. The robustness of these adaptation methods against distribution shifts have not been studied. In this study, we assess the robustness of 11 widely-used adaptation methods across 4 vision-language datasets under multimodal corruptions. Concretely, we introduce 7 benchmark datasets, including 96 visual and 87 textual corruptions, to investigate the robustness of different adaptation methods, the impact of available adaptation examples, and the influence of trainable parameter size during adaptation. Our analysis reveals that: 1) Adaptation methods are more sensitive to text corruptions than visual corruptions. 2) Full fine-tuning does not consistently provide the highest robustness; instead, adapters can achieve better robustness with comparable clean performance. 3) Contrary to expectations, our findings indicate that increasing the number of adaptation data and parameters does not guarantee enhanced robustness; instead it results in even lower robustness. We hope this study could benefit future research in the development of robust multimodal adaptation methods. The benchmark, code, and dataset used in this study can be accessed at https://adarobustness.github.io .

==> check_list.tex <==
\section*{Checklist}

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Supplementary Section 4.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%

\begin{enumerate}

\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See supplementary material}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerYes{See supplementary material}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}

\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerNA{}
	\item Did you include complete proofs of all theoretical results?
    \answerNA{}
\end{enumerate}

\item If you ran experiments (e.g. for benchmarks)...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See supplementary material and \url{https://adarobustness.github.io}}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See supplementary material}
	\item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerNA{}
	\item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See supplementary material}
\end{enumerate}

\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{}
  \item Did you mention the license of the assets?
    \answerYes{See supplementary material}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{See supplementary material}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerYes{See supplementary material}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerYes{See supplementary material}
\end{enumerate}

\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}

\end{enumerate}


==> rebuttal.tex <==
\section{2nd round to Rating 4 (Aug 30)}
Dear reviewer,

thank you very much for your response and we appreciate your acknowledgement of the additional experiments. 

> The contribution claim…
> 
> Suggestion (1): Clarifying the contribution claim to accurately reflect the paper's focus
> 

We agree with this point of view and have **clarified our contribution in the revised version (Line 43)** which limits the research scope to image-language models and tasks. Our work focuses on image-language models and is unrelated to video-language models. Therefore, the suggestion to add more experiments on video-language models may not be applicable to this work. 


> Use existing corruption methods in this work without new corruption methods…
> 
> No new evaluation metric…
>
> Suggestion (2): Introducing new evaluation metrics tailored to this unique task of analyzing the robustness of adaptation methods.
> 

The main objective of this work is to benchmark and analyze the robustness of different adaptation methods, rather than creating new corruption methods or evaluation metrics. 

The NeurIPS Dataset and Benchmark track has accepted several papers [1, 3, 4] that have not provided newly designed perturbation methods or metrics but presented benchmarking experiments with analysis. While designing new methods and metrics is important, **this track also recognizes the value of analysis and benchmarking work, as stated in the track standard**.

This work adopts corruption methods that cover the majority of common image and text perturbation methods widely used in natural robustness research. For example, the text corruptions cover all character, word, and sentence levels and combine methods from various papers [1, 2, 5, 6], resulting in 87 different text perturbations. Additionally, the image corruptions used in this work are standard perturbation settings and are widely adopted in many robustness research studies [1, 2, 7, 8, 9, 10, 11]. 

To study the robustness against these conventional and standard perturbations is **thus necessary and beneficial to the community**. Newly designed corruption methods **cannot replace the study in this work**, and these corruption methods are still needed to draw conclusions, even with a new evaluation metric.



> Suggestion (3):  Conducting additional experiments to establish a more comprehensive and definitive conclusion; 
> 
> Suggestion (4) Providing valuable insights for future research, resulting in a detailed and well-substantiated conclusion, in contrast to the current vague version.
> 

Thanks for your suggestions! Several conclusions have been drawn from our wide range of experiments. 

Based on our discussion and analysis in Section 6.1, we have drawn the following conclusions.

1. Although full fine-tuning generally achieves higher clean performance, its robustness is comparatively weaker than other adaptation methods. The same conclusions can be drawn on corrupted data with different corruption levels.
2. A single adapter can achieve similar or better robustness on VQAv2, NLVR$^2$, and MSCOCO Caption compared to full fine-tuning. On GQA, multiple and half-shared adapters are better. This conclusion applies to both image and text corruptions. 
3. The single-sharing setting could hinder the robustness on certain VL tasks. This applies to Single Adapter, Single LoRA, as well as Single Compacter. 
4. Information sharing with other datasets may hinder the robustness on GQA. To overcome such issues, one can adopt the multiple-module manner or Hyperformer.

The experiment results in Section 6.2 lead to the following conclusions:

1. A potential vulnerability of adaptation methods on multimodal VL models to text corruptions, particularly those at the character level.
2. Among image corruptions, *zoom blur* drops the robustness the most, and within text corruptions, *char-level* methods are most challenging to these VL adaptation methods. These also apply to the compounding scenario. 
3. Language information plays a more significant role than visual information, which also explains the higher sensitivity to text corruptions compared to the sensitivity to image corruptions. 

Analysis in Section 6.3 reveals that

1. Increasing the size of the adaptation data does not consistently enhance relative robustness.
2. More parameters do not ensure enhanced robustness and some even reduce it, such as the single compacter and single adapter on GQA.

We would appreciate **more concrete** advice on which conclusion is not convincing, as well as **corresponding suggestions** for improving the experiment design.

Thanks again for your suggestions and feedback. 

Best regards,

The authors

### References

[1] Robustness analysis of video-language models against visual and language perturbations, NeurIPS 2022

[2] Are multimodal models robust to image and text perturbations? NeurIPS 2022 Workshop DistShift.

[3] Robustness Disparities in Face Detection, NeurIPS 2022

[4] Benchmarking the Robustness of Spatial-Temporal Models Against Corruptions, NeurIPS 2021 

[5] Adversarial GLUE: A Multi-Task Benchmark for Robustness Evaluation of Language Models, NeurIPS 2021 

[6] Textflint: Unified multilingual robustness evaluation toolkit for natural language processing, ACL 2021

[7]  Benchmarking neural network robustness to common corruptions and perturbations. ICLR 2019

[8] Measuring Robustness to Natural Distribution Shifts in Image Classification, NeurIPS 2020

[9] Using Self-Supervised Learning Can Improve Model Robustness and Uncertainty, NeurIPS 2019 

[10] Vision transformers are robust learners, AAAI 2022 

[11] Understanding The Robustness in Vision Transformers, ICML 2022


\section{Summary of the revision and responses}

Dear reviewers,

We would like to express our sincere gratitude for your thoughtful and constructive feedback. We are grateful to see that reviewers find our work essential to the community (Reviewers *Npuc*, *Ssg9* and *rME1*), our findings insightful and beneficial (Reviewers *Npuc*, *Ssg9*, *rME1*, and *gdTB*), our experiments comprehensive (Reviewers *Npuc*, *Ssg9*, *rME1*, *UNok*), and the structure of our paper well-written (Reviewers *Ssg9*, *gdTB*, and *UNok*).

We have considered your feedback and carefully made the following major revisions in the revised version to address your concerns.

1. **New Experiments on Natural Distribution Shifts.** Both Reviewer *Npuc* and Reviewer *gdTB* suggested that including additional natural distribution shifts would be advantageous. Therefore, an additional VQA dataset, **VQA-RAD** [1], from the medical domain has been included in the revised version. A total of **17 new experiments** have been conducted using VQA-RAD on two models. The results are consistent with the findings in the original paper. Concretely, adapters can outperform full-finetuning on both models, especially on CLIP-BART. On CLIP-T5, the best performance is from Multiple Adapters. Full finetuning fails to generalize well in CLIP-BART compared to other adaptation methods. 
2. **New Experiments on Compounding Influence.** Reviewer *rME1* suggested discussing the occurrence of visual and textual corruption together. We agree with this point and have conducted related experiments, discussing their compounding influence. We deployed **a total of 48 new experiments**, including a selection of corruption methods from each category for each modality, as well as two adaptation methods for two models.
    
    As expected, combining corruptions from two modalities can lead to a greater drop in robustness. Besides, the results show similar trends as with single-modal corruptions. Given the same level of image corruption, Character-level corruptions still lead to the most severe performance drop compared to sentence- and word-level corruptions. Zoom blur still reduces robustness the most.
    
3. **Report of Trainable Parameters.** Reviewers *Ssg9* and *gdTB* care about the comparison of the learning efficiency of different adaptation methods. We agree with this point and have added the number of trainable parameters in each adaptation method to Tab. 2 on page 6 of the manuscript.
4. **Revisions on the Paper.** We have made the following additions and changes:
    - Added new experimental results and analysis of natural distribution shifts to Section 6.1 (lines 239-256).
    - Added analysis of compounding effects in Section 6.2 (lines 277-297).
    - Added a new column to the table on page 6 showing the number of trainable parameters.
    - Mentioned the source of images used in this study in the Introduction section (lines 38-40), as suggested by reviewer *Ssg9*.
    - Condensed the original Section 4.2 and included it as a paragraph in Section 5  (lines 189-194), following the suggestions from reviewer *rME1*.

Thank you all again for your time and expertise, and we hope to continue to engage in fruitful discussions with you.

Best regards,

The Authors

### References

[1] A dataset of clinically generated visual questions and answers about radiology images, Scientific data, 2018, 5(1): 1-10.



\section{# Rating 4}
Response to reviewer gdTB (1/3)

Dear reviewer,

Thank you for your feedback and questions. We were grateful to see your acknowledgment of our insightful findings and well-written paper. 

### Regarding the Opportunities For Improvement

> (1) The paper aimed to evaluate the robustness of adaptation models on pre-trained vision-language models, but the evaluation benchmark only focused on image-text models. Therefore, the claim regarding the contribution may be overstated considering the limited scope of the evaluation.
> 

We totally agree that pre-trained vision-language models include more than image-text models. This term is also widely used in the literature on image-text models, such as CLIP-T5[14], Vl-T5[18], MAGMA[19], VisualBERT[16], LXMERT [17], etc. 

We will consider multiple suggestions and ultimately change to a suitable name. We are happy to discuss this issue deeper in the latter rounds!

> (2) ...Therefore, it would be beneficial for the authors to include a performance comparison of learning efficiency alongside the investigation of robustness....
> 

Thanks for pointing this out! 

We agree with this point and have added the percentage of trainable adaptation parameters in each adaptation method to Tab. 2 on page 6, where the larger the number is, the more parameters need to be updated during adaptation. 

The relationship between the number of trainable parameters and the robustness aligns with two of our conclusions. The first is that more parameters do not ensure enhanced robustness and the second is that a single adapter can achieve similar or better robustness compared to full-finetuning despite its much fewer parameters.

> (3) The authors mostly adopted image corruption methods directly from existing sources, with only one addition called "blank." Consequently, the novelty contribution of these corruption methods appears to be insufficient. It would be valuable for the authors to propose new corruption methods that are distinct and allow for a meaningful performance comparison of different adaptation methods.” 
> 
> (6) The text corruption models seem to be directly adopted from existing sources, which diminishes the novelty contribution of these corruption methods. It is recommended that the authors propose new text corruption methods that contribute significantly to the evaluation and comparison of adaptation methods.
> 
> (7) The evaluation metric used in the paper appears to be the same as in previous works [51,4]. To strengthen the novelty contribution of the evaluation metric section, it would be beneficial to propose an alternative robustness evaluation metric specifically designed for assessing adaptation methods.
> 

Thank you for your suggestions. As these three points share similar concerns, we will address them together. 

We acknowledge that most of the corruption methods and metrics used in this study are based on existing works [1, 2, 3]. However, developing novel perturbation methods is actually not the primary goal of this work. Instead, by evaluating the robustness following the most conventional and standard settings, the results can be compared more accurately to existing work [1, 2, 3]. Our work focuses on the robustness of the adaptation method on VLM to common corruption methods. 

More meaningful multimodal perturbation methods are definitely needed for both research and applications, and we leave them to our future work.

> (4) It is essential to evaluate and comprehend whether the choice of different adaptation methods genuinely influences robustness performance. Since the primary learning objective of adaptation methods is not to enhance robustness, it is possible that the robustness performance is primarily dependent on the model itself. Examining this aspect will provide a clearer understanding of the impact of adaptation methods on robustness.
> 

This is a great point and thank the reviewer for pointing this out！

We have also considered such an issue and observed that the robustness of an adaptation method under the same corruption can vary across models. The robustness difference caused by different VL models is also investigated in this work (Sec. 6.1 in Supplementary) and will be moved to the main paper. For instance, all adaptation methods on CLIP-BART had higher robustness against text corruptions on the GQA dataset. 

On the other hand, given a specific VL model, the robustness performance can also show significant gaps between different adaptation methods. For example, the relative robustness varies from 78\% to 89\% on CLIP-T5 given image corruptions on GQA and the relative robustness varies from 73\% to 77\% on CLIP-BART given text corruptions on VQAv2. Overall, different models can lead to different robustness results. But given a specific VL model, different adaptation methods are also able to show distinct robustness.


Response to reviewer gdTB (2/3)

> (5) The image corruption methods mainly consist of synthetic corruptions. To create a comprehensive benchmark, it would be advantageous to include additional natural distribution shifts and adversarial corruptions. This expanded evaluation will provide a more realistic assessment of the model's robustness.
> 

Thanks for your suggestions! 

We agree to this point and have added new experiments on VQA task in the revised version. **VQA-RAD** [1] from the medical domain has been included in the revised version. In the revised version, **17 new experiments** have been conducted on VQA-RAD using two models. The results are consistent with the original paper, showing that adapters can outperform full-finetuning, especially in CLIP-BART. The best performance on CLIP-T5 is also achieved with Multiple Adapters. (Section 6.1 presents a detailed analysis.)

As for the adversarial corruptions, there are quite many different adversarial attacks, such as FGSM [5], PGD [6], MIM [7], and SI [8], etc., against different attacked components, such as input text tokens [9, 10, 12], input images [11], multimodal embeddings [13], and even more adaptive attacks [20], etc. A wide range of experiments have to be conducted in order to draw any solid conclusion, which is impossible given the limited space in this paper. More investigations on the adversarial side are also essential for a realistic assessment of the model’s robustness. We will study this matter in our future work. 

> (8) The paper exclusively employed CLIP-BART (T5) [60] as the base model, which might not be sufficient to draw conclusive findings in the benchmark. It is advisable to evaluate additional architectures to ensure a more convincing and comprehensive conclusion.
> 

Thank you for your suggestions! 

Our work mainly follows the work in VL-Adapter [14] which conducted abundant experiments on hyperparameter tuning for various adaptation methods. We kept the settings the same to ensure the reliability of our experimental results. 

Besides, there is a lack of a solid baseline [15] for other architectures, e.g. VisualBERT [16], LXMERT [17]. To obtain reliable conclusions on other VL models, a wide range of experiments is required to determine the optimal hyperparameter combinations for different tasks, including the information-sharing mechanism in different adapter-based methods, insertion positions for different adaptation modules, and varying hyperparameter combinations. Therefore, it is quite challenging to provide a comprehensive analysis given the limited space in this paper.

> (9) Is there a definitive conclusion regarding the most significant factor influencing robustness? It would be valuable for the authors to provide insights into the primary factors that have a substantial impact on the robustness of adaptation models based on their findings.
> 

Thank you for your question! In our work, we have investigated quite a few influential factors such as corrupted modality, adaptation methods, evaluation tasks, the sharing mechanism,  adaptation data size, adaptation parameter size, hyperparameters, etc. 

From our experiments, we conclude that 1) different corrupted modalities can lead to quite different robustness and text corruptions drop the robustness more than visual corruptions. 2) different evaluation tasks and different sharing mechanisms show different results and should be treated differently. For example, information sharing with other two datasets may hinder the robustness of GQA (Line 250, Sec. 6.1. ). 3) Simply increasing the size of adaptation data and adaptation parameters does not necessarily lead to better robustness. 

> (10) Can the authors present any findings or ideas on how to improve robustness using adaptation methods?
> 

Thank you for your question! We found that adaptation methods are more sensitive to text corruptions. So methods to ensure robustness in LLMs [23] may also be beneficial for adaptation methods on VL models, such as data augmentation [21, 22], and model pretraining [25], etc.

Besides, it is observed that the robustness on GQA may get influenced by the information-sharing mechanism. So one can adopt the multiple-module manner or Hyperformer on GQA to improve robustness. Further investigation into the sharing mechanism is also worthwhile.

Response to reviewer gdTB (3/3)

### Regarding the Limitations section

> (1) It may be unclear whether the selected baseline model is enough to support the claim of the findings.
> 

Our study is based on the work of VL-Adapter [2] which demonstrates competitive adaptation performance compared with full finetuning. VL-Adapter has conducted abundant experiments on hyperparameter tuning for various adaptation methods and we follow the settings to ensure the reliability of our conclusions. 

On the other hand, solid baselines are still missing [15] for other architectures, e.g. VisualBERT [16], LXMERT [17], etc. In order to draw reliable conclusions, a wide range of experiments must be conducted to find the best hyperparameters for each adaptation method on different VL models. The hyperparameters can include the information-sharing mechanism in different adapter-based methods, the insertion positions for different adaptation modules, and the different hyperparameter combinations for different tasks, etc. It is thus difficult to present a thorough analysis given the limited space in this paper.

> (2) Most of the perturbation methods are adopted from existing works directly, the novelty contribution seems trivial. 
(3) The evaluation metric is adopted from previous works as well, no new evaluation metric is proposed.
> 

The primary goal of this study is not to develop new perturbation methods. Instead, the study aimed to evaluate the robustness of the adaptation method on VLM to common corruption methods. Conventional and standard settings ensure more accurate comparisons to existing work [1, 2, 3]. Our future work will focus on developing more perturbation methods specially designed for multimodal models.

Thank you again for your thoughtful and constructive feedback! We hope our response is helpful to address your concerns and you can raise the score for us. 

Yours sincerely, 

The authors

### References

[1] Benchmarking neural network robustness to common corruptions and perturbations, ICLR 2019

[2] Robustness analysis of video-language models against visual and language perturbations, NeurIPS 2022

[3] Are multimodal models robust to image and text perturbations? NeurIPS 2022 Workshop DistShift.

[4] A dataset of clinically generated visual questions and answers about radiology images, Scientific data, 2018, 5(1): 1-10.MLA

[5] Explaining and harnessing adversarial examples[J]. arXiv preprint arXiv:1412.6572, 2014.

[6] Towards deep learning models resistant to adversarial attacks. arXiv preprint arXiv:1706.06083, 2017.

[7] Boosting adversarial attacks with momentum, CVPR 2018

[8] Nesterov accelerated gradient and scale invariance for adversarial attacks, ICLR 2020

[9] Bert-attack: Adversarial attack against bert using bert[J]. arXiv preprint arXiv:2004.09984, 2020.

[10] Generating natural language adversarial examples through probability weighted word saliency, ACL 2019

[11] Fooling vision and language models despite localization and attention mechanism, CVPR 2018

[12] Don't just assume; look and answer: Overcoming priors for visual question answering, CVPR 2018

[13] Towards adversarial attack on vision-language pre-training models, Proceedings of the 30th ACM International Conference on Multimedia. 2022: 5005-5013.

[14] Vl-adapter: Parameter-efficient transfer learning for vision and-language tasks, CVPR 2022

[15]Vision-language pre-training: Basics, recent advances, and future trends, Foundations and Trends in Computer Graphics and Vision, 2022, 14(3–4): 163-352.

[16] Visualbert: A simple and performant baseline for vision and language, arXiv preprint arXiv:1908.03557, 2019.

[17] Lxmert: Learning cross-modality encoder representations from transformers, EMNLP 2019

[18] Unifying vision-and-language tasks via text generation, ICML 2021

[19] MAGMA--Multimodal Augmentation of Generative Models through Adapter-based Finetuning, EMNLP 2022

[20] Obfuscated Gradients Give a False Sense of Security: Circumventing Defenses to Adversarial Examples, ICML 2018

[21] AugMix: A simple data processing method to improve robustness and uncertainty, ICLR 2020

[22] A Survey of Data Augmentation Approaches for NLP, ACL 2021

[23] Measure and Improve Robustness in NLP Models: A Survey, NAACL 2022

[24] An empirical study on robustness to spurious correlations using pre-trained language models, ACL 2020

\section{# Rating 5 }
\subsection{## Response to AC }
Draw attention to a review

Dear Area Chair,

Thank you for handling our paper.

We would like to draw attention to the comments provided by reviewer *UNok* with a confidence score of 5. Despite the high confidence rating, the comments provided by the reviewer **do not make sense at all**. We have three points to highlight our argument.

1. In the Summary and Contributions section, the reviewer makes a misinformed conclusion that "The results show that existing adaptation methods are vulnerable to adversarial attacks." However, our work is **completely unrelated to** adversarial attacks. We believe that the reviewer is either not familiar with this field or has not read our paper. 
2. In the Opportunities for Improvement section, suggestions are not applicable to our work. 
    1. In the first point, the reviewer argues that our method does not consider the semantic alternation caused by text corruption. However, we have already introduced a semantic preserving mechanism used in existing literature [1], [2], in the main paper (line 163), supplementary materials (line 71), and code to ensure that the semantics remain recognizable.
    2. In the second point, the reviewer suggests we add more transferability experiments. However, transferability of attacking methods is again **unrelated to our work**. Our work focuses on the robustness against distribution shifts rather than the adversarial robustness of adaptation methods on VL models. 
3. The same applies to the Limitations section. The reviewer prefers more adversarial attack methods, which are **not our research focus** in this work.

Based on the points mentioned above, we hope AC can take this issue into consideration when making a final recommendation.

Thank you sincerely for your time.

Yours sincerely,

The authors

**References**

[1] Jielin Qiu, Yi Zhu, Xingjian Shi, Florian Wenzel, Zhiqiang Tang, Ding Zhao, Bo Li, and Mu Li. Are multimodal models robust to image and text perturbations? NeurIPS 2022 Workshop DistShift.

[2] Nils Reimers and Iryna Gurevych. Sentence-bert: Sentence embeddings using siamese bert-networks. In EMNLP, 11 2019.

\subsection{## Response to reviewer }
Response to reviewer UNok (1/2)
Dear reviewer,

Thank you very much for your feedback! There may be some incorrect impressions about our topic. Our work focuses on the robustness of adaptation methods on pre-trained vision-language models against **distribution shifts**, rather than adversarial attacks. In other words, our work investigates **natural robustness**, rather than adversarial robustness.

To examine natural robustness, we consider common corruptions, such as different types of noise [1, 2, 3], blurring effects [1, 2, 3], and weather conditions in images [1, 2, 3]. For text, corruptions include typos [2, 3], character modifications [2, 3], back translations [2, 3], and others. There are also many studies on adversarial robustness, which use methods such as Projected Gradient Descent (PGD) [4], CW attack [5], Genetic attack [6], FGSM [9], MIM [10], SI [11], adaptive attacks [12], and feature-level attacks [7], etc.

### Regarding the Opportunities For Improvement

> (1) The text corruptions are not semantic preserving. It's well known that text transforms may break the original semantic meaning of the texts. As shown in the qualitative results in Figure 1, some of the adversarial texts are hard even for humans to understand. Inserting too many chars and typos and dropping the important nouns may make the sentence unclear. As a benchmark easy for people to use, it's better to provide high-quality data and corresponding statistics. It's better to conduct human studies and only include the samples accepted and understandable by humans in the final version of the benchmark since the unacceptable samples are harmful to the models and can not accurately assess the performance of different adaptation methods.
> 

We have also noticed this issue. As stated in Line 162, we introduced a semantic preserving mechanism that is used in existing literature [3,8]. Specifically, we adopt paraphrases from pre-trained sentence-transformers [8] to evaluate the semantic similarity between the original and the corrupted sentences. Detailed information can be found in the code [here](https://github.com/adarobustness/corruption/blob/main/text_corruption/ensure_fidelity.py) where the `paraphrase-mpnet-base-v2` model [8] is used for the cosine similarity calculation. 

> (2) The transferability experiments would be useful when analyzing different attacks and different adaptation methods. For example, some corruption examples are more transferable and may be hard for most of the adaptation methods. These insights are useful for later research in the community.
> 

Thank you for your suggestion. However, please note that transferability experiments, which belong to adversarial attacks, **are not studied in this work**. Therefore, it is not valid to directly add transferability experiments. However, we do plan to study the adversarial robustness of adaptation methods on pre-trained vision-language models, and such transferability experiments would definitely be worth investigating.

> (3). More corruption methods can be included in the experiments. The benchmark only considers visual and textual transformations. More advanced adversarial attack methods can also be interesting.
> 

Thank you for your suggestions! We also believe that robustness against adversarial attacks is essential for developing and deploying adaptation methods on vision-language models. However, due to space constraints, this is not the primary focus of this work and we will focus on this aspect in our future work.

### Regarding the Limitations

> (1) The human study is missing.
> 

We have utilized a widely adopted mechanism [3, 8] to preserve semantic meaning after corruption. This method ensures that the corrupted text has the same semantics as the original one to make sure the image-tex pairs remain meaningful. 


> (2) The attacking strategy is limited. More adversarial attacks can be considered.
> 

Please note that our work does not involve adversarial attacks. Our goal is to investigate the natural robustness of adaptation methods on vision-language models. To this end, we use more than **90 different corruptions**, **including both vision and text modalities**. We believe that the current number of corruption methods is sufficient to draw meaningful conclusions. However, it is indeed essential to examine the adversarial robustness of these adaptation methods, and we will focus on this in our future work.

Thank you for your positive feedback regarding the novelty, comprehensiveness, and presentation of our work. We hope this rebuttal addresses your concerns, and we kindly request that you consider raising the score for our work.

Yours sincerely,

The authors 

Response to reviewer UNok (2/2): References

### References

[1] Dan Hendrycks and Thomas Dietterich. Benchmarking neural network robustness to common corruptions and perturbations. arXiv preprint arXiv:1903.12261, 2019.

[2]  Madeline Chantry, Shruti Vyas, Hamid Palangi, Yogesh Rawat, and Vibhav Vineet. Robustness analysis of video-language models against visual and language perturbations. Advances in Neural Information 320 Processing Systems, 35:34405–34420, 2022.

[3]Jielin Qiu, Yi Zhu, Xingjian Shi, Florian Wenzel, Zhiqiang Tang, Ding Zhao, Bo Li, and Mu Li. Are multimodal models robust to image and text perturbations? arXiv preprint arXiv:2212.08044, 2022.

[4] Aleksander Madry, Aleksandar Makelov, Ludwig Schmidt, Dimitris Tsipras, and Adrian Vladu. Towards deep learning models resistant to adversarial attacks. arXiv preprint arXiv:1706.06083, 2017.

[5]  Carlini, N.; and Wagner, D. 2017. Towards evaluating the robustness of neural networks. In 2017 ieee symposium on security and privacy (sp), 39–57. IEEE

[6]  Alzantot, M.; Sharma, Y.; Elgohary, A.; Ho, B.-J.; Srivastava, M.; and Chang, K.-W. 2018. Generating natural language adversarial examples. arXiv preprint arXiv:1804.07998.

[7] Qiuling Xu, Guanhong Tao, Siyuan Cheng, Lin Tan, and Xiangyu Zhang. Towards feature space adversarial attack. arXiv preprint arXiv:2004.12385, 2020.

[8]  Nils Reimers and Iryna Gurevych. Sentence-bert: Sentence embeddings using siamese bert-networks. In EMNLP, 11 2019.

[9]  Goodfellow I J, Shlens J, Szegedy C. Explaining and harnessing adversarial examples[J]. arXiv preprint arXiv:1412.6572, 2014.

[10] Dong Y, Liao F, Pang T, et al. Boosting adversarial attacks with momentum[C]//Proceedings of the IEEE conference on computer vision and pattern recognition. 2018: 9185-9193.

[11] Lin J, Song C, He K, et al. Nesterov accelerated gradient and scale invariance for adversarial attacks[J]. arXiv preprint arXiv:1908.06281, 2019.

[12] Obfuscated Gradients Give a False Sense of Security: Circumventing Defenses to Adversarial Examples, ICML 2018

\section{# Rating 6  by Ssg9}

Response to reviewer Ssg9 (1/2)

Dear reviewer,

Thank you very much for your thoughtful and constructive review, and for your recognition of the value of this research. We are grateful to read that you find our work very important, very well-written, and insightful. 

### Regarding the Opportunities For Improvement:

> (1) Questionable novelty on the data side.
> 

ImageNet-C [1] is a pioneering work in this field and has inspired this work. In Sections 6.1 and 6.2, we discuss the relationship between the corruption methods introduced in ImageNet-C and the relative robustness of adaptation methods. Additionally, most corrupted images can be seen as a variant of ImageNet-C in the multimodal domain and share the same spirit as they follow the same corruption methods.


> (2) Not clear if the data is available.
> 

Thank you for your interest in our datasets. **All the clean data, corrupted data, pre-trained models, adapted models, and code are publicly available.** We have released the corruption code and benchmark code to the community. The corruption experiments are relatively easy to replicate and we have also released the corrupted datasets. Regarding the [NO] statement in the checklist, we have removed this example statement demo in our revised version to avoid such misunderstanding. More clear instructions now are provided in the paper and our project page. 

> (3) Only one image-text architecture tested.
> 

Thank you for your suggestions and we appreciate your acknowledgement of the wide range of experiments.  This study is based on the work of VL-Adapter [2] which demonstrates competitive adaptation performance compared with full finetuning. Abundant experiments are conducted on hyperparameter tuning for various adaptation methods in VL-Adapter, and we follow the same settings to ensure the reliability of our conclusions. 
Solid baselines are still missing [15] For other architectures, e.g. VisualBERT [16], LXMERT [17], etc. To reach conclusive findings on other VL models, a wide range of experiments must be conducted to determine the best hyperparameters for each adaptation method on different VL models. This includes evaluating the information-sharing mechanism in different adapter-based methods, insertion positions for different adaptation modules, and different hyperparameter combinations for various tasks.  Due to the limited space in this paper, it is challenging to provide a comprehensive analysis.


> (4) Statistical significance of results.
> 

Thank you for your acknowledgment of the expansive experiments. Regarding deviations w.r.t. random initialization of parameters, we have also conducted different initialization methods, such as `uniform`, `xavier_normal` and `kaiming_normal`, and different random initialization seeds.  It turns out that different initialization **do not contribute too much** to the final robustness and we omitted the related analysis in the paper. These minor differences are not reported in our paper and our conclusions are drawn from results showing significant performance gaps. Besides, all the hyperparameters (e.g., learning rates) follow the settings from the original CLIP-T5 [2] to ensure clean performance.

> (5) [Minor issue] Useful information missing from results table.
> 

We acknowledge and appreciate your feedback. We agree with your suggestion and have included information on the percentage of trainable parameters for each adaptation method in Table 2 on page 6 of the revised manuscript.

Response to reviewer Ssg9 (2/2)

### Regarding the Clarity section,

> Only one issue with clarity: the introduction section discusses the number of corruptions introduced by this benchmark, but makes no mention of the source of image. The first time the authors mention these corruptions are added on top of VQAv2, GQA, etc. is in Section 4. I think it should be mentioned earlier. The same applies to text corruptions.
> 

Thanks for pointing this out! We agree with this point and have added the source of the image, and corruption methods earlier in the introduction in the revised version (Line 38-40). 

### Regarding the Relation to Prior Work section,

> This paper has a very comprehensive related work section, that does a good job at putting this work in context and identifying a gap in the literature. It also summarizes very well the adaptation methods used in the experiments.
However, I still don't understand though why ImageNet-C is not part of this benchmark since it inspired all the corruptions used here.
> 

Thank you for acknowledging the comprehensiveness and correctness of the related work section. To address your concerns, our primary goal is to focus on vision-language tasks that involve text generation, such as visual question answering and image captioning. The task settings mainly follow the choices in CLIP-T5 [2] and VL-T5 [3]. While the evaluation of image classification is not well-handled by the CLIP-T5 [2] structure, we plan to add an image classification dataset in our future work.

### Regarding the Documentation section,

> The supplementary provides ample details about the image and text corruption process, with examples.
> 
> 
> The supplementary also includes training details for reproducing the experiments.
> 
> The authors also state that they will “publicize our benchmark datasets, corruption codes, and benchmark codes under MIT License“, which should make it usable to the public. However I am a bit confused because Line 525 of page 14 states that “Did you include the license to the code and datasets? [No] The code and the data are proprietary”.
> 

Thank you for acknowledging our supplementary materials, and we apologize for any misunderstandings. **All clean images, corrupted images, pre-trained models, adapted models, and code are publicly available.** In our revised version, we have removed the example statement you mentioned and provided clearer instructions for the reader.

### Regarding the Additional Feedback

> (1) Is the generated data available or does one have to redo all the work of regenerating the obfuscations?
> 

Yes, the generated corrupted datasets are also publicly available. We also release the corruption code which makes it easier to corrupt other image and text datasets. 

> (2) Why did the authors not experiment with ImageNet-C and other existing image obfuscation datasets? Visual-language models can still be used for image classification. The same question goes for NLP robustness datasets.
> 

The main reason is that we primarily focus on the task setting in the original CLIP-T5 [2] and VL-T5 [3].  The evaluation of image classification is not well-handled by the CLIP-T5 [2] structure but we will support this in future work.

> (3) A suggestion for improvement that can make the paper stronger is including other state-of-the-art vision language models in the experiments, but that is perhaps for future iterations of this paper.
> 

Thank you for your suggestions! We agree with this point and are willing to examine more VL models in our future work.

Thank you again for your review and comments. We hope our response help to address your concerns. 

Best regards,

The authors 

### References 

[1] Dan Hendrycks and Thomas Dietterich. Benchmarking neural network robustness to common corruptions and perturbations. arXiv preprint arXiv:1903.12261, 2019.

[2] Yi-Lin Sung, Jaemin Cho, and Mohit Bansal. Vl-adapter: Parameter-efficient transfer learning for vision and-language tasks. In Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition, pages 5227–5237, 2022

[3] Cho J, Lei J, Tan H, et al. Unifying vision-and-language tasks via text generation[C]//International Conference on Machine Learning. PMLR, 2021: 1931-1942.


\section{# Rating 6 by rME1}
Response to reviewer rME1 

Dear reviewer,

Thank you for reviewing our work and we appreciate your recognition of the value of our work and the effort we put into this project. 

### Regarding the Opportunities for Improvement:

> (1) About significance: is the multimodal robustness significant in VL model adaptation? From Table 2, we can see that the clean accuracy of adaptation methods is still not perfect and the threat of image corruption is not apparent.
> 

We acknowledge that currently, these adaptation methods do not perform as well as full fine-tuning in some cases. The corruptions introduced in this work are relatively common in real-world applications, such as the snowy effects and typos in text. Therefore, the investigation of the robustness against these corruptions is meaningful. Both performance and robustness directions are important and should be considered in research.

> (2) Relative Robustness in Section 4.2 is PO/PI, this section is too long for a simple metric.
> 

We agree with this opinion and have made it more concise in the revised version and put it into a paragraph in Section 5 (Lines 190-195). 

> (3) The submission only discusses the robustness in the test stage. I am curious about what happens to clean accuracy and robustness when the training samples are corrupt.
> 

We appreciate this thought-provoking question. We expect that the robustness will improve as the out-of-distribution examples would have already been shown in the training stage under such circumstances. This exposure can facilitate the testing phase. 

However, we often do not know what kind of distribution shifts will occur in real-world applications and it is impossible to include all possibilities in the training stage to enhance the robustness. Hence, during experiments, the corrupted examples are excluded from the training stage to simulate such scenarios, where the corruptions are unknown to the model during development.

> (4) Authors should discuss when visual corruption and textual corruption appear together.
> 

We agree with this opinion and have added the experiments along with the corresponding analysis to the revised version (Sec. 6.2). In total, we conducted **48 new experiments** across both CLIP-BART and CLIP-T5, using a variety of corruption methods from each modality and two adaptation methods. 

As expected, combining corruptions from two modalities can lead to a greater drop in robustness. Besides, The results show similar trends as with single-modal corruptions. Character-level corruptions still lead to the most severe performance drop compared to sentence- and word-level corruptions. Zoom blur still reduces robustness the most among visual corruptions.

> (5) In Fig. 3, it seems that the robustness of adaptation methods varies a lot between different pre-trained models. Why does this occur, and will the conclusions drawn from the experiment become invalid with the replacement of the pre-trained model?
> 

Thank you for your questions. Fig. 3. presents the relative robustness **against the single blank corruption**. If we consider **the overall robustness averaged across all corruption methods**, as shown in Tab. 5 on the supplementary page 9, the robustness does not vary a lot between different pre-trained models. For example, single adapter has a relative robustness of 85.76\% on CLIP-BART and 85.19\% on CLIP-T5. Although there are still differences between different pre-trained models, our main conclusions remain consistent. For instance, we observe that single adapters can achieve similar or better robustness on VQAv2, NLVR$^2$, and MSCOCO Caption compared to full fine-tuning. This applies to both CLIP-BART and CLIP-T5.


### Regarding the Clarity section

> (1) The paper is overall clear, but figures (e.g., Fig. 4, Fig. 5) should be aligned and presented in a more logical and readable manner.
> 

Thank you for your advice. We have reorganized the order of the figures to make them more logical and readable. 

Thanks again for your time and effort! We hope our response has addressed your concerns.

Best regards,

The authors



\section{# Rating 7  }
Response to reviewer Npuc


Dear reviewer,

Thank you for reviewing our work and recognizing its value. We have put a lot of effort into this project, and we appreciate your acknowledgment!

### Regarding the Opportunities for Improvement

> (1) "...It would be interesting to construct at least one natural distribution shift for VQA and study these same axes."
> 

This is a thoughtful suggestion as domain shifts are also common in real-world applications. We agree with this point and have added one more distribution-shifted test datasets (VQA-RAD [1]) in the revised version. A total of **17 new experiments** have been conducted using VQA-RAD on two models.  The results follow the similar findings in the original paper. For example, adapters have been found to outperform full-finetuning, particularly in the case of CLIP-BART. Full finetuning has been observed to not generalize well in CLIP-BART when compared to other adaptation methods. In CLIP-T5, the best performance is achieved with Multiple Adapters (Check Sec. 6.1 for detailed analysis.)

> (2) "Did the authors conduct a learning rate sweep for their full fine-tuning experiments?" Did the authors do a learning rate sweep for their full fine-tuning experiments? The paper Robust fine-tuning of zero-shot models generally finds that you can get significant robustness improvements by lowering the learning rate significantly during fine-tuning (see the appendix).
> 

Yes, we did. We acknowledge that learning rate is a crucial factor during adaptation, and our current results are based on the best learning rate we found. Different learning rates led to either worse clean performance or longer adaptation times. The paper *Robust fine-tuning of zero-shot models*[2] mainly focuses on different fine-tuning approaches (last-layer vs. end-to-end fine-tuning, hyperparameter changes, etc.), whereas our work primarily examines the robustness of different adaptation methods (prompt tuning, LoRA, adapters, etc.). Therefore, the conclusions may not directly hold in our case.

Thank you again for your constructive feedback and thoughtful comments. We appreciate them greatly. We hope that our response addresses your concerns.

Best regards,

The authors 

### References 

[1] A dataset of clinically generated visual questions and answers about radiology images. Scientific data 2018

[2] Robust fine-tuning of zero-shot models, CVPR 2022

==> sections/z-old_analysis.tex <==
\section{Results and Analysis}








%\textbf{Adapter, Compacter and Hyperformer}


% \textbf{VQA}

% \textbf{Captioning} 

% \textbf{GQA}
% Single adaptation methods on text are neither good. Single Lora, Single Compacter, Single Adapter 

% \textbf{NLVR}

% \textbf{Combination of tasks}



%\textbf{Image Corruption Methods by Category}
% a figure showing the results on several methods 

%\textbf{Text Corruption Methods by Category}

% a figure showing the results on char-level 

% \textbf{Multimodal Compounding Robustness.} As VL tasks deal with both visual and language information, to understand the compounding effects of distribution shift in both visual and language domain is also important. We have selected a subset of corruption methods from the main category in both image and text data and conducted robustness evaluation on them. >>>>TODO>>>>

%\subsection{The relationship between adaptation parameter size and robustness}



% \subsection{Robustness of Model Adaptation on various VL models}
% CLIP-BART
% CLIP-T5
% CLIP-ViL (discriminative)
% BLIP2 (single stream)


==> sections/z-old_tables.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{\label{BART-img-corr-avg} Relative Robustness of BART against img corruptions (avg on 5 severities).}
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Adaptation method} & \textbf{VQA}      & \textbf{GQA}      & \textbf{NLVR}     & \textbf{Caption}  \\ \midrule
Full Finetuning            & 0.918 $\pm$ 0.043 & 0.940 $\pm$ 0.030 & 0.950 $\pm$ 0.029 & 0.835 $\pm$ 0.094 \\
Multiple Adapters          & 0.920 $\pm$ 0.042 & 0.909 $\pm$ 0.029 & 0.962 $\pm$ 0.025 & 0.839 $\pm$ 0.094 \\
Half-shared Adapters       & 0.919 $\pm$ 0.042 & 0.941 $\pm$ 0.030 & 0.958 $\pm$ 0.024 & 0.836 $\pm$ 0.093 \\
Single Adapter             & 0.927 $\pm$ 0.043 & 0.875 $\pm$ 0.031 & 0.948 $\pm$ 0.029 & 0.836 $\pm$ 0.093 \\
Hyperformer                & 0.920 $\pm$ 0.041 & 0.948 $\pm$ 0.029 & 0.944 $\pm$ 0.025 & 0.836 $\pm$ 0.092 \\
Multiple Compacters        & 0.922 $\pm$ 0.041 & 0.936 $\pm$ 0.029 & 0.956 $\pm$ 0.026 & 0.837 $\pm$ 0.093 \\
Single Compacter           & 0.920 $\pm$ 0.041 & 0.875 $\pm$ 0.031 & 0.962 $\pm$ 0.024 & 0.847 $\pm$ 0.091 \\
Multiple LoRA              & 0.915 $\pm$ 0.042 & 0.955 $\pm$ 0.027 & 0.983 $\pm$ 0.008 & 0.837 $\pm$ 0.093 \\
Single LoRA                & 0.915 $\pm$ 0.042 & 0.873 $\pm$ 0.029 & 0.945 $\pm$ 0.027 & 0.839 $\pm$ 0.090 \\
Single Prompt              & 0.954 $\pm$ 0.023 & 0.959 $\pm$ 0.020 & 0.993 $\pm$ 0.006 & 0.835 $\pm$ 0.093 \\
Multiple Prompts           & 0.949 $\pm$ 0.026 & 0.958 $\pm$ 0.024 & 0.995 $\pm$ 0.002 & 0.829 $\pm$ 0.094 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\centering
\caption{\label{BART-img-corr-avg} Relative Robustness of BART against img corruptions (severity 5).}
\begin{tabular}{@{}cllll@{}}
\toprule
\textbf{Adaptation method} & \multicolumn{1}{c}{\textbf{VQA}} & \multicolumn{1}{c}{\textbf{GQA}} & \multicolumn{1}{c}{\textbf{NLVR}} & \multicolumn{1}{c}{\textbf{Caption}} \\ \midrule
Full Finetuning            & 0.849$\pm$0.052                  & 0.892$\pm$0.038                  & 0.903$\pm$0.037                   & 0.684$\pm$0.139                      \\
Multiple Adapters          & 0.853$\pm$0.049                  & 0.862$\pm$0.042                  & 0.920$\pm$0.042                   & 0.687$\pm$0.137                      \\
Half-shared Adapters       & 0.852$\pm$0.050                  & 0.894$\pm$0.040                  & 0.917$\pm$0.038                   & 0.684$\pm$0.141                      \\
Single Adapter             & 0.858$\pm$0.053                  & 0.825$\pm$0.044                  & 0.900$\pm$0.047                   & 0.687$\pm$0.135                      \\
Hyperformer                & 0.854$\pm$0.048                  & 0.900$\pm$0.038                  & 0.901$\pm$0.045                   & 0.687$\pm$0.138                      \\
Multiple Compacters        & 0.857$\pm$0.048                  & 0.889$\pm$0.039                  & 0.913$\pm$0.044                   & 0.687$\pm$0.134                      \\
Single Compacter           & 0.855$\pm$0.050                  & 0.826$\pm$0.042                  & 0.920$\pm$0.043                   & 0.699$\pm$0.132                      \\
Multiple LoRA              & 0.848$\pm$0.049                  & 0.911$\pm$0.037                  & 0.975$\pm$0.012                   & 0.685$\pm$0.140                      \\
Single LoRA                & 0.848$\pm$0.048                  & 0.826$\pm$0.042                  & 0.900$\pm$0.045                   & 0.693$\pm$0.133                      \\
Single Prompt              & 0.916$\pm$0.029                  & 0.928$\pm$0.030                  & 0.981$\pm$0.013                   & 0.686$\pm$0.131                      \\
Multiple Prompts           & 0.908$\pm$0.036                  & 0.919$\pm$0.036                  & 0.991$\pm$0.007                   & 0.677$\pm$0.135                      \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{\label{BART-text-corr-avg} Relative Robustness of CLIP-BART against text corruptions (avg on 5 severities).}
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{Adaptation method} & VQA               & GQA               & NLVR              \\ \midrule
Full Finetuning            & 0.793 $\pm$ 0.039 & 0.723 $\pm$ 0.043 & 0.895 $\pm$ 0.018 \\
Multiple Adapters          & 0.815 $\pm$ 0.035 & 0.719 $\pm$ 0.039 & 0.924 $\pm$ 0.017 \\
Half-shared Adapters       & 0.818 $\pm$ 0.035 & 0.736 $\pm$ 0.043 & 0.914 $\pm$ 0.017 \\
Single Adapter             & 0.827 $\pm$ 0.035 & 0.722 $\pm$ 0.036 & 0.909 $\pm$ 0.018 \\
Hyperformer                & 0.801 $\pm$ 0.035 & 0.754 $\pm$ 0.040 & 0.898 $\pm$ 0.019 \\
Multiple Compacters        & 0.819 $\pm$ 0.034 & 0.726 $\pm$ 0.041 & 0.922 $\pm$ 0.016 \\
Single Compacter           & 0.822 $\pm$ 0.034 & 0.728 $\pm$ 0.036 & 0.923 $\pm$ 0.016 \\
Multiple LoRA              & 0.789 $\pm$ 0.035 & 0.740 $\pm$ 0.041 & 1.002 $\pm$ 0.000 \\
Single LoRA                & 0.796 $\pm$ 0.036 & 0.688 $\pm$ 0.038 & 0.902 $\pm$ 0.018 \\
Single Prompt              & 0.806 $\pm$ 0.024 & 0.767 $\pm$ 0.031 & 1.001 $\pm$ 0.000 \\
Multiple Prompts           & 0.837 $\pm$ 0.025 & 0.811 $\pm$ 0.030 & 1.004 $\pm$ 0.000 \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{\label{BART-text-corr-5} Relative Robustness of CLIP-BART against text corruptions (severity 5).}
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{Adaptation method} & VQA             & GQA             & NLVR            \\ \midrule
Full Finetuning            & 0.737$\pm$0.224 & 0.669$\pm$0.241 & 0.871$\pm$0.110 \\
Multiple Adapters          & 0.766$\pm$0.207 & 0.669$\pm$0.224 & 0.901$\pm$0.102 \\
Half-shared Adapters       & 0.768$\pm$0.208 & 0.682$\pm$0.248 & 0.892$\pm$0.101 \\
Single Adapter             & 0.776$\pm$0.211 & 0.675$\pm$0.200 & 0.885$\pm$0.109 \\
Hyperformer                & 0.751$\pm$0.213 & 0.703$\pm$0.231 & 0.873$\pm$0.113 \\
Multiple Compacters        & 0.771$\pm$0.208 & 0.674$\pm$0.233 & 0.900$\pm$0.098 \\
Single Compacter           & 0.772$\pm$0.204 & 0.679$\pm$0.203 & 0.901$\pm$0.098 \\
Multiple LoRA              & 0.740$\pm$0.220 & 0.688$\pm$0.228 & 1.002$\pm$0.008 \\
Single LoRA                & 0.745$\pm$0.214 & 0.639$\pm$0.210 & 0.876$\pm$0.110 \\
Single Prompt              & 0.770$\pm$0.190 & 0.725$\pm$0.203 & 1.001$\pm$0.005 \\
Multiple Prompts           & 0.802$\pm$0.172 & 0.771$\pm$0.165 & 1.004$\pm$0.005 \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]\centering
\caption{\label{T5-img-corr-avg} Relative Robustness of T5 against img corruptions (avg on 5 severities).}
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Adaptation method} & \textbf{VQA}      & \textbf{GQA}      & \textbf{NLVR}     & \textbf{Caption}  \\ \midrule
Full Finetuning            & 0.918 $\pm$ 0.042 & 0.922 $\pm$ 0.030 & 0.942 $\pm$ 0.030 & 0.842 $\pm$ 0.092 \\
Multiple Adapters          & 0.922 $\pm$ 0.042 & 0.921 $\pm$ 0.027 & 0.985 $\pm$ 0.007 & 0.830 $\pm$ 0.095 \\
Single Adapter             & 0.919 $\pm$ 0.042 & 0.832 $\pm$ 0.029 & 0.937 $\pm$ 0.030 & 0.837 $\pm$ 0.093 \\
Hyperformer                & 0.926 $\pm$ 0.040 & 0.936 $\pm$ 0.026 & 0.955 $\pm$ 0.026 & 0.851 $\pm$ 0.090 \\
Single Compacter           & 0.923 $\pm$ 0.041 & 0.854 $\pm$ 0.030 & 0.948 $\pm$ 0.030 & 0.842 $\pm$ 0.092 \\
Multiple Compacters        & 0.923 $\pm$ 0.040 & 0.925 $\pm$ 0.027 & 0.969 $\pm$ 0.014 & 0.830 $\pm$ 0.093 \\ \bottomrule
\end{tabular}
\end{table}


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]\centering
\caption{\label{T5-img-corr-avg} Relative Robustness of T5 against img corruptions (severity 5).}
\begin{tabular}{@{}cllll@{}}
\toprule
\textbf{Adaptation method} & \multicolumn{1}{c}{\textbf{VQA}} & \multicolumn{1}{c}{\textbf{GQA}} & \multicolumn{1}{c}{\textbf{NLVR}} & \multicolumn{1}{c}{\textbf{Caption}} \\ \midrule
Full Finetuning            & 0.851$\pm$0.051                  & 0.875$\pm$0.040                  & 0.894$\pm$0.043                   & 0.693$\pm$0.138                      \\
Multiple Adapters          & 0.855$\pm$0.048                  & 0.877$\pm$0.039                  & 0.974$\pm$0.019                   & 0.676$\pm$0.146                      \\
Single Adapter             & 0.852$\pm$0.052                  & 0.786$\pm$0.040                  & 0.887$\pm$0.050                   & 0.685$\pm$0.140                      \\
Hyperformer                & 0.860$\pm$0.049                  & 0.893$\pm$0.039                  & 0.911$\pm$0.046                   & 0.705$\pm$0.135                      \\
Single Compacter           & 0.856$\pm$0.051                  & 0.806$\pm$0.042                  & 0.900$\pm$0.043                   & 0.692$\pm$0.139                      \\
Multiple Compacters        & 0.859$\pm$0.049                  & 0.881$\pm$0.040                  & 0.948$\pm$0.016                   & 0.680$\pm$0.137                      \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{\label{T5-text-corr-avg} Relative Robustness of T5 against text corruptions (avg on 5 severities).}
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{Adaptation method} & VQA               & GQA               & NLVR              \\ \midrule
Full Finetuning            & 0.750 $\pm$ 0.072 & 0.648 $\pm$ 0.087 & 0.874 $\pm$ 0.034 \\
Multiple Adapters          & 0.769 $\pm$ 0.062 & 0.631 $\pm$ 0.085 & 0.994 $\pm$ 0.002 \\
Single Adapter             & 0.769 $\pm$ 0.063 & 0.631 $\pm$ 0.067 & 0.872 $\pm$ 0.035 \\
Hyperformer                & 0.770 $\pm$ 0.059 & 0.682 $\pm$ 0.081 & 0.888 $\pm$ 0.031 \\
Single Compacter           & 0.769 $\pm$ 0.064 & 0.637 $\pm$ 0.070 & 0.887 $\pm$ 0.029 \\
Multiple Compacters        & 0.775 $\pm$ 0.062 & 0.678 $\pm$ 0.077 & 1.001 $\pm$ 0.001 \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{\label{T5-text-corr-5} Relative Robustness of T5 against text corruptions (severity 5).}
\begin{tabular}{@{}clll@{}}
\toprule
\textbf{Adaptation method} & \multicolumn{1}{c}{VQA} & \multicolumn{1}{c}{GQA} & \multicolumn{1}{c}{NLVR} \\ \midrule
Full Finetuning            & 0.725$\pm$0.253         & 0.643$\pm$0.258         & 0.877$\pm$0.107          \\
Multiple Adapters          & 0.767$\pm$0.212         & 0.623$\pm$0.259         & 0.994$\pm$0.009          \\
Single Adapter             & 0.759$\pm$0.212         & 0.633$\pm$0.194         & 0.878$\pm$0.107          \\
Hyperformer                & 0.765$\pm$0.208         & 0.670$\pm$0.244         & 0.891$\pm$0.101          \\
Single Compacter           & 0.762$\pm$0.212         & 0.642$\pm$0.202         & 0.887$\pm$0.099          \\
Multiple Compacters        & 0.764$\pm$0.211         & 0.677$\pm$0.227         & 1.000$\pm$0.003          \\ \bottomrule
\end{tabular}
\end{table}

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]\centering
\tiny
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}ccccccccccccccccccccccc@{}}
\toprule
\textbf{Adaptation method} & \textbf{Clean} & \textbf{Impulse} & \textbf{Gaussian} & \textbf{Shot} & \textbf{Speckle} & \textbf{Zoom} & \textbf{Defocus} & \textbf{Motion} & \textbf{Glass} & \textbf{Gaussian} & \textbf{JPEG} & \textbf{Contrast} & \textbf{Elastic} & \textbf{Pixelate} & \textbf{Snow} & \textbf{Frost} & \textbf{Fog} & \textbf{Brightness} & \textbf{Spatter} & \textbf{Saturate} & \textbf{ave} & \textbf{ave relative robustness} \\ \midrule
Full Finetuning            & 115.03         & 81.17                  & 81.35                   & 85.44               & 94.18                  & 37.14              & 86.8                  & 75.71                & 65.06               & 83.06                  & 101.57                    & 64.22             & 71.91                      & 62.17             & 72.51         & 71.96          & 84.94        & 105.19              & 72               & 98.52             & 78.68            & 0.684                            \\
Multiple Adapters          & 114.47         & 80.382                 & 80.15                   & 83.148              & 93.494                 & 38.745             & 86.249                & 76.844               & 67.18               & 83.254                 & 101.351                   & 63.33             & 71.333                     & 60.88             & 71.467        & 73.985         & 85.879       & 105.201             & 73.135           & 98.585            & 78.66            & 0.687                            \\
Half-shared Adapters       & 114.5          & 79.944                 & 79.987                  & 84.561              & 93.942                 & 36.509             & 85.722                & 75.587               & 66.158              & 82.142                 & 100.892                   & 62.498            & 72.542                     & 60.165            & 72.11         & 72.363         & 85.265       & 105.799             & 74.231           & 98.81             & 78.38            & 0.685                            \\
Single Adapter             & 115.038        & 80.804                 & 79.906                  & 84.103              & 94.777                 & 39.022             & 86.771                & 76.413               & 67.248              & 82.81                  & 100.003                   & 63.395            & 72.09                      & 62.762            & 72.54         & 73.265         & 86.301       & 105.832             & 74.194           & 99.028            & 79.01            & 0.687                            \\
Hyperformer                & 114.868        & 81.486                 & 81.184                  & 84.695              & 94.778                 & 38.876             & 87.22                 & 77.358               & 65.7                & 83.811                 & 100.726                   & 63.684            & 71.187                     & 61.52             & 72.182        & 72.184         & 86.937       & 105.541             & 72.977           & 98.137            & 78.96            & 0.687                            \\
Multiple Compacters        & 115.16         & 80.384                 & 81.337                  & 84.001              & 93.927                 & 40.35              & 86.581                & 77.254               & 66.264              & 83.457                 & 100.487                   & 64.146            & 72.046                     & 61.457            & 71.873        & 73.236         & 87.801       & 105.852             & 73.753           & 98.307            & 79.08            & 0.687                            \\
Single Compacter           & 113.06         & 81.779                 & 80.075                  & 83.994              & 93.597                 & 42.833             & 85.97                 & 77.867               & 67.299              & 82.556                 & 99.625                    & 63.003            & 71.916                     & 60.521            & 71.843        & 74.022         & 87.75        & 104.961             & 74.435           & 97.933            & 79.05            & 0.699                            \\
Multiple LoRA              & 115.407        & 80.405                 & 80.375                  & 84.802              & 94.76                  & 37.083             & 87.011                & 77.123               & 67.137              & 83.624                 & 100.765                   & 63.069            & 71.88                      & 60.501            & 72.661        & 73.329         & 87.289       & 106.065             & 74.051           & 99.355            & 79.01            & 0.685                            \\
Single LoRA                & 114.543        & 81.349                 & 81.511                  & 85.88               & 93.202                 & 41.466             & 85.975                & 76.136               & 67.718              & 82.823                 & 100.427                   & 64.944            & 72.111                     & 61.093            & 72.42         & 73.498         & 87.241       & 105.519             & 74.293           & 99.632            & 79.33            & 0.693                            \\
Single Prompt              & 103.7          & 72.487                 & 72.331                  & 75.718              & 84.932                 & 40.531             & 76.78                 & 70.319               & 58.32               & 73.44                  & 89.506                    & 58.412            & 64.682                     & 52.919            & 64.575        & 66.29          & 78.047       & 95.558              & 66.092           & 89.98             & 71.1             & 0.686                            \\
Multiple Prompts           & 108.619        & 75.508                 & 74.45                   & 78.38               & 87.429                 & 41.641             & 81.407                & 72.983               & 59.526              & 77.612                 & 92.618                    & 58.532            & 65.953                     & 53.735            & 65.299        & 68.627         & 80.86        & 100.67              & 67.949           & 93.914            & 73.53            & 0.677                            \\ \bottomrule
\end{tabular}}
\end{table}

\begin{table}[]
\centering
\caption{\label{BARTvst5-img-corr-level-5} BART vs T5 given img corruption (severity 5).}
\begin{tabular}{@{}ccccc@{}}
\toprule
\textbf{Adaptation method} & \textbf{VQA} & \textbf{GQA} & \textbf{NLVR} & \textbf{Caption} \\ \midrule
Full finetuning & T5 & BART & BART & T5 \\
Multiple adapters & T5 & T5 & T5 & BART \\
Single adapter & BART & BART & BART & BART (almost the same) \\
Hyperformer & T5 & BART & T5 & T5 \\
Single compacter & T5 (almost the same) & BART & BART & BART \\
Multiple compacters & T5 & BART & T5 & BART \\ \bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\centering
\caption{\label{BARTvst5-text-corr-level-5} BART vs T5 given text corruption (severity 5).}
\begin{tabular}{@{}cccc@{}}
\toprule
\textbf{Adaptation method} & \textbf{VQA} & \textbf{GQA} & \textbf{NLVR} \\ \midrule
Full finetuning & BART & BART & almost the same \\
Multiple adapters & almost the same & BART & T5 \\
Single adapter & BART & BART & BART \\
Hyperformer & T5 & BART & T5 \\
Single compacter & BART & BART & BART \\
Multiple compacters & BART & almost the same & T5 \\ \bottomrule
\end{tabular}
\end{table}


\begin{table}[]
\centering
\caption{\label{BART-img-corr-level-vqa-5} VQA Relative Robustness of CLIP-BART against img corruptions (severity 5).}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}ccccccccccccccc@{}}
\toprule
\textbf{Adaptation method} & \textbf{Clean} & \textbf{Noise} & \textbf{Noise RR} & \textbf{Blur} & \textbf{Blur RR} & \textbf{Digital} & \textbf{Digital RR} & \textbf{Weather} & \textbf{Weather RR} & \textbf{Spatter} & \textbf{Spatter RR} & \textbf{Saturate} & \textbf{Saturate RR} & \textbf{Ave RR} \\ \midrule
Full finetuning & 66.75 & 57.41 & 0.86 & 55.56 & 0.832 & 55.6 & 0.833 & 57.56 & 0.862 & 55.8 & 0.836 & 60.41 & 0.905 & 0.849 \\
Multiple adapters & 65.3 & 56.33 & 0.863 & 55.03 & 0.843 & 54.68 & 0.837 & 56.37 & 0.863 & 54.88 & 0.84 & 59.13 & 0.906 & 0.853 \\
Half shared adapters & 65.2 & 56.04 & 0.86 & 54.62 & 0.838 & 54.66 & 0.838 & 56.28 & 0.863 & 55.03 & 0.844 & 59.13 & 0.907 & 0.852 \\
Single adapter & 65.35 & 56.77 & 0.869 & 54.93 & 0.841 & 55.14 & 0.844 & 56.96 & 0.872 & 54.93 & 0.841 & 59.71 & 0.914 & 0.858 \\
Hyperformer & 65.38 & 56.45 & 0.863 & 54.98 & 0.841 & 54.98 & 0.841 & 56.5 & 0.864 & 54.89 & 0.84 & 59.13 & 0.904 & 0.854 \\
Multiple compacters & 64.91 & 56.06 & 0.864 & 54.72 & 0.843 & 54.81 & 0.844 & 56.42 & 0.869 & 54.7 & 0.843 & 58.81 & 0.906 & 0.856 \\
Single compacter & 64.47 & 55.82 & 0.866 & 54.15 & 0.84 & 54.08 & 0.839 & 55.92 & 0.867 & 54.37 & 0.843 & 58.54 & 0.908 & 0.855 \\
Multiple lora & 65.44 & 56.13 & 0.858 & 54.64 & 0.835 & 54.64 & 0.835 & 56.13 & 0.858 & 54.47 & 0.832 & 58.83 & 0.899 & 0.848 \\
Single lora & 65.34 & 55.9 & 0.856 & 54.5 & 0.834 & 54.56 & 0.835 & 56.15 & 0.859 & 54.6 & 0.836 & 58.92 & 0.902 & 0.848 \\
Single prompt & 44 & 40.66 & 0.924 & 40.04 & 0.91 & 40.06 & 0.91 & 40.48 & 0.92 & 39.81 & 0.905 & 41.28 & 0.938 & 0.916 \\
Multiple prompts & 46.81 & 43.17 & 0.922 & 42.23 & 0.902 & 42.09 & 0.899 & 42.25 & 0.903 & 42.18 & 0.901 & 44.08 & 0.942 & 0.908 \\ \bottomrule
\end{tabular}}
\end{table}

\begin{table}[]
\centering
\scriptsize
\caption{\label{BART-text-corr-level-vqa-5} VQA Relative Robustness of CLIP-BART against text corruptions (severity 5).}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}ccccccccc@{}}
\toprule
\textbf{Adaptation method} & \textbf{Clean} & \textbf{Char-level} & \textbf{Char-level RR} & \textbf{Word-level} & \textbf{Word-level RR} & \textbf{Sentence-level} & \textbf{Sentence-level RR} & \textbf{Ave RR} \\ \midrule
Full finetuning            & 66.75          & 32.33               & 0.484                  & 51.99               & 0.779                  & 64.68                   & 0.969                      & 0.736           \\
Multiple adapters          & 65.3           & 33.76               & 0.517                  & 53.21               & 0.815                  & 63.55                   & 0.973                      & 0.766           \\
Half shared adapters       & 65.2           & 33.75               & 0.518                  & 53.28               & 0.817                  & 63.48                   & 0.974                      & 0.768           \\
Single adapter             & 65.35          & 33.65               & 0.515                  & 54.42               & 0.833                  & 63.83                   & 0.977                      & 0.776           \\
Hyperformer                & 65.38          & 33.52               & 0.513                  & 51.6                & 0.789                  & 63.69                   & 0.974                      & 0.751           \\
Multiple compacters        & 64.91          & 33.63               & 0.518                  & 53.38               & 0.822                  & 63.27                   & 0.975                      & 0.771           \\
Single compacter           & 64.47          & 33.76               & 0.524                  & 53.12               & 0.824                  & 62.25                   & 0.966                      & 0.772           \\
Multiple lora              & 65.44          & 33.51               & 0.512                  & 50.53               & 0.772                  & 63.66                   & 0.973                      & 0.74            \\
Single lora                & 65.34          & 32.89               & 0.503                  & 51.27               & 0.785                  & 63.41                   & 0.97                       & 0.745           \\
Single prompt              & 44             & 28.89               & 0.657                  & 33.49               & 0.761                  & 42.75                   & 0.972                      & 0.77            \\
Multiple prompts           & 46.81          & 29.35               & 0.627                  & 38.88               & 0.831                  & 45.4                    & 0.97                       & 0.802           \\ \bottomrule
\end{tabular}}
\end{table}



\begin{table}[]
\centering
\scriptsize
\caption{\label{BART-img-corr-level-nlvr-5} NLVR Relative Robustness of CLIP-BART against img corruptions (severity 5).}
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}ccccccccccccccc@{}}
\toprule
\textbf{Adaptation method} & \textbf{Clean} & \textbf{Noise} & \textbf{Noise RR} & \textbf{Blur} & \textbf{Blur RR} & \textbf{Digital} & \textbf{Digital RR} & \textbf{Weather} & \textbf{Weather RR} & \textbf{Spatter} & \textbf{Spatter RR} & \textbf{Saturate} & \textbf{Saturate RR} & \textbf{Ave RR} \\ \midrule
Full finetuning & 73.01 & 66.31 & 0.908 & 66.3 & 0.908 & 64.55 & 0.884 & 66.42 & 0.91 & 65.81 & 0.901 & 66.75 & 0.914 & 0.903 \\
Multiple adapters & 69.41 & 64.36 & 0.927 & 63.21 & 0.911 & 62.94 & 0.907 & 64.96 & 0.936 & 64.03 & 0.922 & 64.46 & 0.929 & 0.92 \\
Half shared adapters & 70.03 & 64.7 & 0.924 & 63.37 & 0.905 & 63.66 & 0.909 & 65.25 & 0.932 & 64.58 & 0.922 & 64.59 & 0.922 & 0.917 \\
Single adapter & 73.89 & 67.42 & 0.912 & 64.89 & 0.878 & 65.81 & 0.891 & 68.07 & 0.921 & 66.28 & 0.897 & 68.18 & 0.923 & 0.9 \\
Hyperformer & 72.21 & 65.96 & 0.913 & 63.86 & 0.884 & 64.13 & 0.888 & 66.34 & 0.919 & 65.49 & 0.907 & 66.07 & 0.915 & 0.901 \\
Multiple compacters & 69.45 & 64.44 & 0.928 & 62 & 0.893 & 62.58 & 0.901 & 64.72 & 0.932 & 63.84 & 0.919 & 64.39 & 0.927 & 0.913 \\
Single compacter & 69.94 & 65.45 & 0.936 & 63.31 & 0.905 & 63.21 & 0.904 & 65.52 & 0.937 & 64.58 & 0.923 & 65.28 & 0.933 & 0.92 \\
Multiple lora & 51.32 & 49.66 & 0.968 & 49.66 & 0.968 & 50.02 & 0.975 & 50.34 & 0.981 & 50.95 & 0.993 & 50.91 & 0.992 & 0.974 \\
Single lora & 73.58 & 67.33 & 0.915 & 65.08 & 0.884 & 64.93 & 0.882 & 67.51 & 0.918 & 66.37 & 0.902 & 68.04 & 0.925 & 0.901 \\
Single prompt & 51.95 & 50.63 & 0.975 & 51.64 & 0.994 & 50.48 & 0.972 & 50.96 & 0.981 & 50.7 & 0.976 & 50.98 & 0.981 & 0.981 \\
Multiple prompts & 49.87 & 49.27 & 0.988 & 49.41 & 0.991 & 49.67 & 0.996 & 49.31 & 0.989 & 49.56 & 0.994 & 49.66 & 0.996 & 0.991 \\ \bottomrule
\end{tabular}}
\end{table}


==> sections/z-removed.tex <==
% Our benchmark analysis concludes that adaptation methods are sensitive to multimodal corruptions such as zoom blur image corruption and especially to character-level text corruptions, e.g. character replacement.

% Multimodal vision-language models have gained significant attention in recent years and have been highly successful in numerous tasks, such as image captioning \cite{li2022mplug, wang2022unifying, li2023blip}, visual question answering \cite{wang2022image, wang2022unifying, bao2022vlmo}, and visual reasoning \cite{wang2022image, zeng2022x}. However, their computational cost is quite high, making it almost impossible for most end users to train a model from scratch or  fully fine-tune a pre-trained foundation model. 

%semantic modification \cite{gardner2020evaluating}, grammar errors \cite{wang-etal-2021-textflint}, dialects \cite{demszky2020learning}, different domains \cite{miller2020effect}, and bias \cite{de2019bias}

% On the other hand, researchers have demonstrated that it is possible to attain comparable performance by optimizing a few parameters \cite{sung2022vladapter, li2021prefix, lester2021prompt}. Therefore, parameter-efficient adaptation methods have been extensively adopted to apply pre-trained large foundation models to a specific setting or a new dataset. Nevertheless, the robustness of these parameter-efficient adaptation methods against distribution shifts is not thoroughly explored. A comprehensive understanding of the robustness of different adaptation methods can help users choose a reliable approach to adapt a complex vision-language model to a new scenario.

% Intro 逻辑如下
% Popularity of Pre-VLM. To improve their performance in a target domain, various model adaptation methods have been proposed
% In real-world applications, the test inputs are often shifted from training-data distributions. robustness against the distribution shift is important . e.g. unexpected wrong decisions are acceptable, e.g. self-driving systems, medical domain
% It is not clear which adaptation method performs better in which tasks. In this work, we benchmark ... 
% Concretely, we include ... corruption and ... dataset. we conclude that ...
% We also release the datasets, test code, and evaluation protocol for benchmarking future adaptation methods 
% Contribution Summarization


% Abstrat 逻辑和 introduction 逻辑 一致 只是每一点一句话总结， intro里面把每一点扩成一小段

% 其他任何 section 都这为了这个逻辑服务 任何一句话都是（什么时候强调什么内容）

% such as UNIMO \cite{li2020unimo} and CLIP \cite{radford2021learning}

% , such as Frozen \cite{tsimpoukelli2021multimodal}, MAGMA \cite{eichenberg2021magma} and Flamingo \cite{alayrac2022flamingo}

% Frozen \cite{tsimpoukelli2021multimodal} trains a vision encoder and projects the input images to visual features that can be understood by the language model. MAGMA \cite{eichenberg2021magma} inserts adapters, whereas Flamingo \cite{alayrac2022flamingo} injects cross-attention layers into the frozen LM.

%  such as VisualBERT \cite{li2019visualbert}, VL-BERT \cite{su2019vl} and LXMERT \cite{tan2019lxmert}
% Cross-stream models \cite{lu2019vilbert, li2021align, tan2019lxmert} encode visual and language information independently using encoder modules, and fuse the different modal information with mutual attention mechanisms. ViLBERT \cite{lu2019vilbert} is a cross-stream model that encodes text and image separately and utilizes two transformers to further model intra-modality interaction after the cross-modal module. ALBEF \cite{li2021align} follows a similar idea and utilizes two separate transformers for images and texts before modality interaction. 

% . Single-stream models \cite{li2019visualbert, su2019vl, cho2021vlt5} integrate language and visual information at the beginning of the model structure.  

 % CLIP \cite{radford2021learning} uses a dual encoder structure with two single-modal encoders to encode images and text separately. CLIP utilizes a straightforward method to map image and text embeddings to the same space for similarity computation and shows surprising performance on several VL tasks.

% Some have analyzed the robustness against color and texture transformations \cite{geirhos2018imagenet, yun2019cutmix, cubuk2019autoaugment}.
%  research has shown that around two-thirds of real-world NLP systems fail after deployment due to the lack of robustness \cite{ribeiro2020beyond}. 
%  Hendrycks et al. \cite{hendrycks2020pretrained} studied the out-of-distribution generalization ability of various models, such as CNNs, LSTMs, and Transformers, on seven NLP datasets.

%Regarding the robustness of transformer-based architectures, Paul et al. showed in \cite{paul2022vision} that vision transformers (ViTs) \cite{dosovitskiy2020vit} are more robust learners against common corruptions, distribution shifts, and natural adversarial examples. Gu et al. found in \cite{gu2022vision} that ViTs are more robust to naturally corrupted patches than CNNs but more vulnerable to adversarial patches.

%Previous studies  have shown that corrupted data can significantly degrade model performance.\cite{geirhos2018generalisation, hendrycks2019benchmarking, geirhos2018imagenet}
%  such as CheckList \cite{ribeiro2020beyond}, WildNLP \cite{rychalska2019models}, TextFlint \cite{wang-etal-2021-textflint}, and Robustness Gym \cite{goel2021robustness}

%such as ImageNet-C, ImageNet-P \cite{hendrycks2019benchmarking}, Stylized-ImageNet \cite{geirhos2018imagenet}, ImageNet-O, and Imagenet-A \cite{hendrycks2021natural}, and ImageNet-V2 \cite{recht2019imagenet}.

%  However, these models are typically designed for a specific task and suffer from poor transferability \cite{du2022survey}.
% These models can be categorized into two categories: single-stream models and cross-stream models \cite{zhou2023comprehensive}
% Vision and language are two essential modalities in our world. 

%Vision-language (VL) tasks consider both visual and linguistic contexts, e.g. image captioning \cite{vinyals2016show} and visual question answering (VQA) \cite{antol2015vqa}. Deep-learning-based models \cite{aneja2018convolutional, lu2018neural, rennie2017self, liu2021cptr, zhang2021rstnet} have shown relatively good performance. 

%  The robustness of multimodal models is harder to evaluate because of more corruption possibilities \cite{chantry2022robustness}.

% Robustness against distribution shift is a requirement when applying machine learning models in real-world scenarios, particularly for high-stakes tasks.

% a b Some work introduced single modality adversarial perturbations to multimodal fusion models \cite{yang2021defending}. \cite{tian2021can} evaluated the robustness of audio-visual models through adversarial attacks on audio, visual, and both modalities. MultiBench \cite{liang2021multibench} is proposed as a general benchmark on learning multimodal representations.

 %\cite{cho2022dall} explored the reasoning skills and robustness against bias of text-to-image generative models.
 
 %about the robustness of existing adaptation methods on vision-language models.

==> sections/z-some-conclusions.tex <==
\subsection{10 conclusions from the original paper}

1. Half-shared adapters perform on par with Multiple Adapters with fewer parameters 

half-shared adapters' robustness is on par with multiple adapters and on GQA, half-shared adapters are better than multiple adapters with fewer parameters. 

2. Single Adapter’s performance is as competitive as which of the full fine-tuning 

On GQA, full-finetuning is more robust than single adapter against image perturbation. 
On other three tasks, single adapter is comparable to full-finetuning. 

3. Information sharing benefits the low resource tasks 


4. Compare to Adapter, Compacter does not stand out in our experiments. because BART is trained on language tasks and the downstream task is VL tasks 
    
    
5. Single Adapter still achieves a promising accuracy-efficiency tradeoff in T5 


6. Prompt-tuning does not perform well in our experiments due to dissimilar pre-trained and downstream tasks 


7. There is only 1\% improvement with adding the CLIP into training, the advantage of adding adapters inside CLIP over keeping it frozen is limited 


8. Freezing BART and only fine-tuning CLIP is far from updating BART suggesting that fine-tuning the LM is crucial 


9. Only updating $\theta ^{V\rightarrow L}$ produces insufficient results, suggesting the need to update the language model partially 


10. Single Adapter is more competitive than full fine-tuning with only a few parameters being trained, suggesting that the adapters work well with different kinds of pre-trained weights 


11. For CLIP-VIL, inserting single adapter to ViL is also effective

==> sections/z-taxonomy.tex <==
full fine-tuning

multimodal

visual question answering 

